Uncertainty in the era of machine learning for atomistic modeling

The widespread adoption of machine learning surrogate models has significantly improved the scale and complexity of systems and processes that can be explored accurately and efficiently using atomistic modeling. However, the inherently data-driven nature of machine learning models introduces uncertainties that must be quantified, understood, and effectively managed to ensure reliable predictions and conclusions. Building upon these premises, in this Perspective, we first overview state-of-the-art uncertainty estimation methods, from Bayesian frameworks to ensembling techniques, and discuss their application in atomistic modeling. We then examine the interplay between model accuracy, uncertainty, training dataset composition, data acquisition strategies, model transferability, and robustness. In doing so, we synthesize insights from the existing literature and highlight areas of ongoing debate.

==> cover.tex <==
[Your Name]
[Your Institution]
[Your Address]
[Your Email Address]
[Your Phone Number]

[Date]

Dear Editorial team,

We are pleased to submit our manuscript titled "Uncertainty in the Era of Machine Learning for Atomistic Modeling" for consideration in Digital Discovery (following preliminary discussions with Alexander Whiteside, Assistant Editor, Digital Discovery). 

This work arises from an international collaboration involving Universita' di Modena e Reggio Emilia, EPFL, NOMATEN, Universita' la Statale di Milano, and TU Delft. This manuscript is an outcome of the DAEMON Network (Data-driven Applications towards the Engineering of functional Materials: an Open Network) funded by COST (European Cooperation in Science and Technology), under the auspices of the European Union.

The adoption of machine learning is determining a paradigm shift in the utility and scale of atomistic modeling for materials discovery and design, enabling the study of complex systems with unprecedented accuracy and efficiency. 
The data-driven nature of machine learning models introduces uncertainties that must be addressed to ensure reliable predictions. 

Building on this premises, this perspective reviews state-of-the-art uncertainty estimation methods, such as Bayesian frameworks and ensemble techniques, and their applications in atomistic modeling.
Further, it examines the relationships between model accuracy, uncertainty, dataset composition, data acquisition, transferability, and robustness. Our goal is to demonstrate how uncertainty quantification can support the development of reliable and transferable machine learning models for materials and molecular sciences, synthesizing insights from recent literature and highlighting ongoing debates.

Given the growing importance of machine learning in atomistic simulations with the end goal of impactful fundamental and application advancements in the context of chemistry, materials science, and physics, we believe this perspective will be of significant interest to your readership. It provides a timely and critical assessment of uncertainty quantification strategies, offering practical guidance and stimulating further discussion within the field.

We confirm that this manuscript has not been submitted elsewhere and has been approved by all authors for submission. Thank you for considering our work, and we look forward to your feedback.


If suitable, as potential reviewers of this manuscript, we would suggest:

Ondrej Marsalek - Charles University

Christoph Schran - University of Cambridge

Daniel Schwalbe-Koda - UCLA

Julia Zavadlav - TUM

Danny Perez - Los Alamos National Laboratory


Sincerely,
[Your Name]
[Your Position/Title]
[Your Institution]
[Your Contact Information]

==> other_files/active_learning.tex <==
“Learn on the Fly”: A Hybrid Classical and Quantum-Mechanical Molecular Dynamics Simulation -  Gabor Csányi, T. Albaret, M. C. Payne, and A. De Vita,  Phys. Rev. Lett. 93, 175503 (2004)

Active learning of linearly parametrized interatomic potentials - Evgeny V. Podryabinkin, Alexander V. Shapeev, Computational Materials Science 140, 171-180 (2017)

Molecular Dynamics with On-the-Fly Machine Learning of Quantum-Mechanical Forces - Zhenwei Li, James R. Kermode, and Alessandro De Vita; Phys. Rev. Lett. 114, 096405 (2015)

On-the-Fly Active Learning of Interatomic Potentials for Large-Scale Atomistic Simulations - Ryosuke Jinnouchi, Kazutoshi Miwa, Ferenc Karsai, Georg Kresse, and Ryoji Asahi, J. Phys. Chem. Lett. 2020, 11, 17, 6946–6955
Computational Materials Science Volume 242, June 2024, 113074 - Active learning for SNAP interatomic potentials via Bayesian predictive uncertainty; Logan Williams a, Khachik Sargsyan a, Andrew Rohskopf b, Habib N. Najm a


Prediction of formation energies of large-scale disordered systems via active-learning-based executions of ab initio local-energy calculations: A case study on a Fe random grain boundary model with millions of atoms
Tomoyuki Tamura and Masayuki Karasuyama
Phys. Rev. Materials 4, 113602 – Published 5 November 2020

Active learning with moment tensor potentials to predict material properties: Ti0.5Al0.5N at elevated temperature featured
F. Bock  ; F. Tasnádi  ; I. A. Abrikosov 

Outlier-Detection for Reactive Machine Learned Potential Energy Surfaces
Luis Itza Vazquez-Salazar, Silvan Käser, Markus Meuwly
arxiv 2024

Computational Materials Science Volume 242, June 2024, 113074 - Active learning for SNAP interatomic potentials via Bayesian predictive uncertainty; Logan Williams a, Khachik Sargsyan a, Andrew Rohskopf b, Habib N. Najm a

Active Learning and Uncertainty Estimation
Chapter (part of Machine Learning Meets Quantum Physics
); 04 June 2020 ; pp 309–329
CAlexander Shapeev, Konstantin Gubaev, Evgenii Tsymbalov & Evgeny Podryabinkin 
%https://link.springer.com/chapter/10.1007/978-3-030-40245-7_15

Simulating Diffusion Properties of Solid-State Electrolytes via a Neural Network Potential: Performance and Training Scheme - Dr. Aris Marcolongo, Dr. Tobias Binninger, Dr. Federico Zipoli, Dr. Teodoro Laino
ChemSysChem -  Volume2, Issue3 ;May 2020 ; e1900031

Transferable Force Field for Gallium Nitride Crystal Growth from the Melt Using On-The-Fly Active Learning ; 
Xiangyu Chen, William Shao, Nam Q. Le, and Paulette Clancy ; J. Chem. Theory Comput. 2023, 19, 21, 7861–7872

========

Local Bayesian optimizer for atomic structures
Estefanía Garijo del Río, Jens Jørgen Mortensen, and Karsten Wedel Jacobsen
Phys. Rev. B 100, 104103 – Published 5 September 2019

Quality of uncertainty estimates from neural network potential ensembles
Leonid Kahle and Federico Zipoli
Phys. Rev. E 105, 015311 – Published 21 January 2022

Error-Controlled Exploration of Chemical Reaction Networks with Gaussian Processes
Gregor N. Simm and Markus Reiher*
Cite this: J. Chem. Theory Comput. 2018, 14, 10, 5238–5248

Self-Parametrizing System-Focused Atomistic Models
Christoph Brunken and Markus Reiher*
Cite this: J. Chem. Theory Comput. 2020, 16, 3, 1646–1665

========

